Controlling the Mutation in Large Language Models for the Efficient Evolution of Algorithms

The integration of Large Language Models (LLMs) with evolutionary computation (EC) has introduced a promising paradigm for automating the design of metaheuristic algorithms. However, existing frameworks, such as the Large Language Model Evolutionary Algorithm (LLaMEA), often lack precise control over mutation mechanisms, leading to inefficiencies in solution space exploration and potentially suboptimal convergence. This paper introduces a novel approach to mutation control within LLM-driven evolutionary frameworks, inspired by theory of genetic algorithms. Specifically, we propose dynamic mutation prompts that adaptively regulate mutation rates, leveraging a heavy-tailed power-law distribution to balance exploration and exploitation. Experiments using GPT-3.5-turbo and GPT-4o models demonstrate that GPT-3.5-turbo fails to adhere to the specific mutation instructions, while GPT-4o is able to adapt its mutation based on the prompt engineered dynamic prompts. Further experiments show that the introduction of these dynamic rates can improve the convergence speed and adaptability of LLaMEA, when using GPT-4o. This work sets the starting point for better controlled LLM-based mutations in code optimization tasks, paving the way for further advancements in automated metaheuristic design.

==> code-diff-mutation.tex <==
\begin{figure}[htp]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-3.5-turbo_2_code-diff.png}
    \caption{gpt-3.5-turbo with requesting $2\%$ mutation rate}
    \label{fig:gpt-3.5-turbo_2_code-diff}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-4o_2_code-diff.png}
    \caption{gpt-4o with requesting $2\%$ mutation rate}
    \label{gpt-4o_2_code-diff}
  \end{subfigure}

  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-3.5-turbo_5_code-diff.png}
    \caption{gpt-3.5-turbo with requesting $5\%$ mutation rate}
    \label{fig:gpt-3.5-turbo_5_code-diff}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-4o_5_code-diff.png}
    \caption{gpt-4o with requesting $5\%$ mutation rate}
    \label{gpt-4o_5_code-diff}
  \end{subfigure}

  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-3.5-turbo_10_code-diff.png}
    \caption{gpt-3.5-turbo with requesting $10\%$ mutation rate}
    \label{fig:gpt-3.5-turbo_10_code-diff}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-4o_10_code-diff.png}
    \caption{gpt-4o with requesting $10\%$ mutation rate}
    \label{gpt-4o_10_code-diff}
  \end{subfigure}

  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-3.5-turbo_20_code-diff.png}
    \caption{gpt-3.5-turbo with requesting $20\%$ mutation rate}
    \label{fig:gpt-3.5-turbo_20_code-diff}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-4o_20_code-diff.png}
    \caption{gpt-4o with requesting $20\%$ mutation rate}
    \label{gpt-4o_20_code-diff}
  \end{subfigure}
\end{figure}


\begin{figure}[htp]
\ContinuedFloat
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-3.5-turbo_40_code-diff.png}
    \caption{gpt-3.5-turbo with requesting $40\%$ mutation rate}
    \label{fig:gpt-3.5-turbo_40_code-diff}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-4o_40_code-diff.png}
    \caption{gpt-4o with requesting $40\%$ mutation rate}
    \label{gpt-4o_40_code-diff}
  \end{subfigure}

  \caption{Influence of Different Prompts on Code Difference Distribution}
  \label{fig:code-diff-mutation}
\end{figure}


==> code-diff-prompts.tex <==
\begin{figure}[htp]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt1_gpt-3.5-turbo_code-diff.png}
    \caption{gpt-3.5-turbo with prompt1}
    \label{fig:prompt1-gpt-3.5-turbo-diff}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt1_gpt-4o_code-diff.png}
    \caption{gpt-4o with prompt1}
    \label{fig:prompt1-gpt-4o-diff}
  \end{subfigure}
  
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt2_gpt-3.5-turbo_code-diff.png}
    \caption{gpt-3.5-turbo with prompt2}
    \label{fig:prompt2-gpt-3.5-turbo-diff}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt2_gpt-4o_code-diff.png}
    \caption{gpt-4o with prompt2}
    \label{fig:prompt2-gpt-4o-diff}
  \end{subfigure}
  
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt3_gpt-3.5-turbo_code-diff.png}
    \caption{gpt-3.5-turbo with prompt3}
    \label{fig:prompt3-gpt-3.5-turbo-diff}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt3_gpt-4o_code-diff.png}
    \caption{gpt-4o with prompt3}
    \label{fig:prompt3-gpt-4o-diff}
  \end{subfigure}
  
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt4_gpt-3.5-turbo_code-diff.png}
    \caption{gpt-3.5-turbo with prompt4}
    \label{fig:prompt4-gpt-3.5-turbo-diff}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt4_gpt-4o_code-diff.png}
    \caption{gpt-4o with prompt4}
    \label{fig:prompt4-gpt-4o-diff}
  \end{subfigure}
\end{figure}


\begin{figure}[htp]
\ContinuedFloat
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt5_gpt-3.5-turbo_code-diff.png}
    \caption{gpt-3.5-turbo with prompt5}
    \label{fig:prompt5-gpt-3.5-turbo-diff}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt5_gpt-4o_code-diff.png}
    \caption{gpt-4o with prompt5}
    \label{fig:prompt5-gpt-4o-diff}
  \end{subfigure}
  
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt6_gpt-3.5-turbo_code-diff.png}
    \caption{gpt-3.5-turbo with prompt6}
    \label{fig:prompt6-gpt-3.5-turbo-diff}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt9_gpt-4o_code-diff.png}
    \caption{gpt-4o with prompt9}
    \label{fig:prompt9-gpt-4o-diff}
  \end{subfigure}
  
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt7_gpt-3.5-turbo_code-diff.png}
    \caption{gpt-3.5-turbo with prompt7}
    \label{fig:prompt7-gpt-3.5-turbo-diff}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt10_gpt-4o_code-diff.png}
    \caption{gpt-4o with prompt10}
    \label{fig:prompt10-gpt-4o-diff}
  \end{subfigure}
  
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt8_gpt-3.5-turbo_code-diff.png}
    \caption{gpt-3.5-turbo with prompt8}
    \label{fig:prompt8-gpt-3.5-turbo-diff}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt11_gpt-4o_code-diff.png}
    \caption{gpt-4o with prompt11}
    \label{fig:prompt11-gpt-4o-diff}
  \end{subfigure}
  \caption{Code Difference Distribution of Different Prompts}
  \label{fig:code-diff-prompts}
\end{figure}


==> mse.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{MSE of delivered/requested.}
\label{tab:mse}
\begin{tabular}{@{}ccccccc@{}}
\toprule
\multirow{2}{*}{model}         & \multirow{2}{*}{prompt} & \multicolumn{5}{c}{requested mutation rates}                                   \\
                               &                         & 2\%            & 5\%           & 10\%          & 20\%          & 40\%          \\ \midrule
\multirow{8}{*}{gpt-3.5-turbo} & prompt1                 & 250.98         & 17.65         & 6.54          & 0.63          & 0.36          \\
                               & prompt2                 & 138.11         & 8.08          & 2.26          & 0.74          & 0.6           \\
                               & prompt3                 & 253.32         & \textbf{7.5}  & 10.88         & 0.82          & 0.53          \\
                               & prompt4                 &                & 13.78         & \textbf{2.06} & 1.16          & 0.38          \\
                               & prompt5                 & \textbf{10.28} &               & 6.77          & \textbf{0.46} & \textbf{0.27} \\
                               & prompt6                 & 547.24         & 53.68         & 7.6           & 1.51          & 0.48          \\
                               & prompt7                 & 317.07         & 48.64         & 8.52          & 1.01          & 0.26          \\
                               & prompt8                 & 173.32         & 37.52         & 14.26         & 1.07          & 0.42          \\ \midrule
\multirow{8}{*}{gpt-4o}        & prompt1                 & 30.44          & 3.97          & 1.92          & 0.65          & 0.3           \\
                               & prompt2                 & 13.97          & 5.35          & \textbf{1.29} & 0.76          & 0.27          \\
                               & prompt3                 & 19.43          & 4.8           & 1.93          & \textbf{0.65} & 0.22          \\
                               & prompt4                 & 35.4           & 3.31          & 2.64          & 0.8           & 0.25          \\
                               & prompt5                 & \textbf{7.49}  & \textbf{0.92} & 1.98          & 0.82          & 0.43          \\
                               & prompt9                 & 155.06         & 16.51         & 3.85          & 1.27          & 0.26          \\
                               & prompt10                & 54.14          & 4.82          & 5.66          & 1.66          & \textbf{0.2}  \\
                               & prompt11                & 375.98         & 40.25         & 4.65          & 1.21          & 0.22          \\ \bottomrule
\end{tabular}
\end{table}

==> ratio-mutation.tex <==
\begin{figure}[htp]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-3.5-turbo_2_ratio.png}
    \caption{gpt-3.5-turbo with requesting $2\%$ mutation rate}
    \label{fig:gpt-3.5-turbo_2_ratio}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-4o_2_ratio.png}
    \caption{gpt-4o with requesting $2\%$ mutation rate}
    \label{gpt-4o_2_ratio}
  \end{subfigure}

  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-3.5-turbo_5_ratio.png}
    \caption{gpt-3.5-turbo with requesting $5\%$ mutation rate}
    \label{fig:gpt-3.5-turbo_5_ratio}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-4o_5_ratio.png}
    \caption{gpt-4o with requesting $5\%$ mutation rate}
    \label{gpt-4o_5_ratio}
  \end{subfigure}

  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-3.5-turbo_10_ratio.png}
    \caption{gpt-3.5-turbo with requesting $10\%$ mutation rate}
    \label{fig:gpt-3.5-turbo_10_ratio}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-4o_10_ratio.png}
    \caption{gpt-4o with requesting $10\%$ mutation rate}
    \label{gpt-4o_10_ratio}
  \end{subfigure}

  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-3.5-turbo_20_ratio.png}
    \caption{gpt-3.5-turbo with requesting $20\%$ mutation rate}
    \label{fig:gpt-3.5-turbo_20_ratio}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-4o_20_ratio.png}
    \caption{gpt-4o with requesting $20\%$ mutation rate}
    \label{gpt-4o_20_ratio}
  \end{subfigure}
\end{figure}


\begin{figure}[htp]
\ContinuedFloat
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-3.5-turbo_40_ratio.png}
    \caption{gpt-3.5-turbo with requesting $40\%$ mutation rate}
    \label{fig:gpt-3.5-turbo_40_ratio}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/gpt-4o_40_ratio.png}
    \caption{gpt-4o with requesting $40\%$ mutation rate}
    \label{gpt-4o_40_ratio}
  \end{subfigure}

  \caption{Influence of Different Prompts on Code Difference Distribution}
  \label{fig:ratio-mutation}
\end{figure}


==> ratio-prompts.tex <==
\begin{figure}[htp]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt1_gpt-3.5-turbo_ratio.png}
    \caption{gpt-3.5-turbo with prompt1}
    \label{fig:prompt1-gpt-3.5-turbo-ratio}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt1_gpt-4o_ratio.png}
    \caption{gpt-4o with prompt1}
    \label{fig:prompt1-gpt-4o-ratio}
  \end{subfigure}
  
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt2_gpt-3.5-turbo_ratio.png}
    \caption{gpt-3.5-turbo with prompt2}
    \label{fig:prompt2-gpt-3.5-turbo-ratio}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt2_gpt-4o_ratio.png}
    \caption{gpt-4o with prompt2}
    \label{fig:prompt2-gpt-4o-ratio}
  \end{subfigure}
  
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt3_gpt-3.5-turbo_ratio.png}
    \caption{gpt-3.5-turbo with prompt3}
    \label{fig:prompt3-gpt-3.5-turbo-ratio}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt3_gpt-4o_ratio.png}
    \caption{gpt-4o with prompt3}
    \label{fig:prompt3-gpt-4o-ratio}
  \end{subfigure}
  
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt4_gpt-3.5-turbo_ratio.png}
    \caption{gpt-3.5-turbo with prompt4}
    \label{fig:prompt4-gpt-3.5-turbo-ratio}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt4_gpt-4o_ratio.png}
    \caption{gpt-4o with prompt4}
    \label{fig:prompt4-gpt-4o-ratio}
  \end{subfigure}
\end{figure}


\begin{figure}[htp]
\ContinuedFloat
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt5_gpt-3.5-turbo_ratio.png}
    \caption{gpt-3.5-turbo with prompt5}
    \label{fig:prompt5-gpt-3.5-turbo-ratio}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt5_gpt-4o_ratio.png}
    \caption{gpt-4o with prompt5}
    \label{fig:prompt5-gpt-4o-ratio}
  \end{subfigure}
  
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt6_gpt-3.5-turbo_ratio.png}
    \caption{gpt-3.5-turbo with prompt6}
    \label{fig:prompt6-gpt-3.5-turbo-ratio}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt9_gpt-4o_ratio.png}
    \caption{gpt-4o with prompt9}
    \label{fig:prompt9-gpt-4o-ratio}
  \end{subfigure}
  
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt7_gpt-3.5-turbo_ratio.png}
    \caption{gpt-3.5-turbo with prompt7}
    \label{fig:prompt7-gpt-3.5-turbo-ratio}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt10_gpt-4o_ratio.png}
    \caption{gpt-4o with prompt10}
    \label{fig:prompt10-gpt-4o-ratio}
  \end{subfigure}
  
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt8_gpt-3.5-turbo_ratio.png}
    \caption{gpt-3.5-turbo with prompt8}
    \label{fig:prompt8-gpt-3.5-turbo-ratio}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{code_diff/prompt11_gpt-4o_ratio.png}
    \caption{gpt-4o with prompt11}
    \label{fig:prompt11-gpt-4o-ratio}
  \end{subfigure}
  \caption{Ratio of Delivered Code Difference to Requested Mutation Rate of Different Prompts, y-axis values is scaled by $\log{10}$.}
  \label{fig:ratio-prompts}
\end{figure}

